AdaChain: A Learned Adaptive Blockchain

This paper presents AdaChain, a learning-based blockchain framework that adaptively chooses the best permissioned blockchain architecture in order to optimize effective throughput for dynamic transaction workloads. AdaChain addresses the challenge in the Blockchain-as-a-Service (BaaS) environments, where a large variety of possible smart contracts are deployed with different workload characteristics. AdaChain supports automatically adapting to an underlying, dynamically changing workload through the use of reinforcement learning. When a promising architecture is identified, AdaChain switches from the current architecture to the promising one at runtime in a way that respects correctness and security concerns. Experimentally, we show that AdaChain can converge quickly to optimal architectures under changing workloads, significantly outperform fixed architectures in terms of the number of successfully committed transactions, all while incurring low additional overhead.

==> response.tex <==
\begin{center}
{\huge \textbf{Response to Reviewer Comments}}
\end{center}

\bigskip

We would like to thank the anonymous reviewers for their thoughtful and constructive feedback. We have significantly revised the paper to address the reviewers' questions and suggestions. 
In this revised paper, we have made low-level changes to many parts of the paper to improve the presentation, but we have only highlighted significant changes in \new{blue} for better readability. Whenever figures are updated, we highlight the corresponding captions. Additionally, for reviewers' reference, we have attached a delta version at the end of this document that also shows deletions, where texts that are removed due to reorganization are shown in \remove{brown}.

In our response below, for each comment, we first summarize how we have addressed it and then point to the specific paragraphs in the revised paper.


\medskip
\noindent
{\large \textbf{Meta-Reviewer}}

\begin{itemize}
    \item \textbf{M1. Give a clear motivation of reinforcement learning. }
    
    \hspace{8pt} We have provided a clear motivation for reinforcement learning. Please refer to our response to Reviewer 2 (C1) for details.
    
    \item \textbf{M2. Discuss the new challenges/novelty of the studied problem in the context of permissioned blockchain comparing to the existing works in DB and system literature.}

    \hspace{8pt} We have discussed how \sys contributes to existing works in configuration prediction and system migration. Please refer to our response to Reviewer 3 (W1) for details.
    
    \item \textbf{M3. Discuss the threat/risks introduced by the configuration switch and migration. }
    
    \hspace{8pt} We have discussed the threats introduced by learning and architecture switch as well as how \sys addresses them. Please refer to our response to Reviewer 3 (W2) and Section 6 for details.

    \item \textbf{M4. Discuss the possibility of providing hints to the learning framework to improve the learning efficiency. }

    \hspace{8pt} We have discussed and evaluated the possibility of providing hints. Please refer to our response to Reviewer 3 (W4) for details.

    \item \textbf{M5. Justify the robustness of choosing the median values. }

    \hspace{8pt} We have justified the robustness of the median values. Please refer to our response to Reviewer 1 (W3) for details.

    \item \textbf{M6. Provide justification of choosing the throughput as the metric to optimize.  }

    \hspace{8pt} We have justified why we choose throughput as the metric to optimize. Please refer to our response to Reviewer 3 (W5) for details.

    \item \textbf{M7. Provide details on how learning agents avoid malicious learning agents from influencing the learning or decision process. }

    \hspace{8pt} We have described the measurement exchange and distributed decision making process in more details. Please refer to our response to Reviewer 3 (W6) for details.

    \item \textbf{M8. Discuss the security of using Thompson sampling. }

    \hspace{8pt} We have discussed the security of Thompson sampling. Please refer to our response to Reviewer 3 (W7) for details.

    \item \textbf{M9. Provide appropriate experiments or explanations to the following questions: 1) the time cost of learning the workload/ideal architecture; 2) What happens if the workload keeps changing at a faster rate; 3) What happens if there are delays in committing the architecture?  }

    \hspace{8pt} We have provided evaluation results or explanations to answer the questions above, as suggested by Reviewer 1 (W1 and W2). Please refer to our responses to these comments for details.
    

    
\end{itemize}

\medskip
\noindent
{\large \textbf{Reviewer 1}}


\begin{itemize}
    \item \textbf{W1. How much time does it typically take to learn the workload/ideal architecture? What happens if the workload keeps changing at a faster rate?}

    \begin{enumerate}
    \item  We have updated {\bf \color{blue}Table~\ref{tbl:avg_tp} and Section~\ref{sec:expstatic}} to show the typical time it takes to learn the best architecture under each workload, i.e., the convergence time. In our definition, convergence is reached when \sys stayed within $95\%$ of the optimal performance for $5$ consecutive episodes.

    \item  Ideally, since we use the state of the previous episode to approximate the state of the next episode, \sys can adapt to workloads that shift less frequently than every two episodes ($20$s at most). In practice, due to the exploration performed by CMAB, as long as the changes are slower than the convergence (as shown in Table~\ref{tbl:avg_tp}), AdaChain operates effectively. We have updated {\bf \color{blue}Section~\ref{sec:expchanging}} to reflect the explanation above.
    \end{enumerate}

    
       
    \item \textbf{W2. I think of “committing the architecture” as a meta-transaction. What happens if there are delays in just committing this meta-transaction? As an adversary, it seems like an obvious target if I have to hurt the performance of the system.}

    \hspace{8pt} We thank the reviewer for pointing out this threat.
    We discuss two cases.
    First, when the adversary delays its own communication (sending messages) during architecture switching.
    In this scenario, if the adversary is a backup node, it does not hurt the system’s throughput assuming the number of faulty backups is no more than $f$.
    On the other hand, if the adversary is the leader, it could carry out a performance attack such as the pre-prepare delay, i.e., delay transition into the new architecture but without triggering the timeout. Fortunately, there are known orthogonal techniques to mitigate these attacks. For example, instead of using a pessimistic switching protocol (inspired by PBFT), we can adopt a robust switching protocol, e.g., following the Prime protocol~\cite{amir2011prime} which is a BFT consensus protocol robust to performance attacks.
    We leave this as future work.

    \hspace{8pt} Second, we next consider an extreme scenario where an adversary is strong enough to somehow delay correct nodes. 
    \sys assumes the partially synchrony model where there exists a global stabilization time (GST), after which all messages between correct replicas are received within some bound $\Delta$. This means honest nodes cannot be delayed indefinitely. Even if we remove this partial synchrony assumption, correctness is always still guaranteed at the expense of some performance degradation. We also note that such attacks are not specific to \sys. In a fixed blockchain architecture, such timing-based attacks are also possible (e.g. adversaries delay messages in the ordering phase), and \sys does not exacerbate this attack. The threat and discussion above are reflected in {\bf \color{blue}Section~\ref{sec:security}}.

    
    
    
    \item \textbf{W3. I am not sure if choosing the median is robust enough. Let’s imagine that we have f honest parties that have a very slow network — this can typically make those parties make incorrect decisions wrt the throughput/how well the existing architecture is performing. The f Byzantine parties can provide incorrect information about this. If the leader is Byzantine, it is required to pick 2f+1 values, out of which 2f would correspond to the slow honest and Byzantine parties. The median would correspond to one of them too?}

    \hspace{8pt} We appreciate the suggestion of justifying the robustness of choosing median values. \sys is designed to operate in a homogeneous environment, where each participating node has similar amounts of compute, memory, storage, and network resources. In this environment, if the $f$ dishonest nodes report false local measurements that are outliers (e.g., infinity or zero), they will be effectively ignored by computing the median since the remaining $f+1$ nodes report honest measurements that are close to each other. Thus, the situation mentioned in this comment is not likely to happen. We provided this explanation in {\bf \color{blue}Section~\ref{sec:security}}.
    
    \hspace{8pt} However, to comprehensively understand the robustness of the median value, we perform an analysis below in a heterogeneous setting: we assume $f+1$ fast honest nodes, $f$ very slow honest nodes, and $f$ Byzantine nodes.

    \begin{enumerate}
        \item If the leader is not malicious:
        \begin{enumerate}
            \item If the $f$ slow honest nodes are caused by a slow network:
            \begin{itemize}
                \item If the $f$ Byzantine nodes attack consensus by delaying communication, then each of the $3f+1$ nodes will have poor throughput measurements due to the latency of the ordering phase (establishing consensus among nodes). In this case, the median is robust.

                \item If the $f$ Byzantine nodes do not attack consensus (i.e., participate in consensus like non-faulty nodes), then the $f+1$ fast honest nodes have high throughput, while the $f$ slow honest nodes might have poor throughput (e.g., fall behind and were not able to process all transactions). When the leader gathers the $2f+1$ quorum needed for switching, the CHECKPOINT message from the $f+1$ fast honest node will first arrive at the leader and be included in the quorum, since their network is faster. In this case, the median value is robust.
            \end{itemize}

            \item If the $f$ slow honest nodes are caused by poor processing power (and/or limited memory):
            \begin{itemize}
                \item The $f$ slow honest nodes would have low throughput measurements due to transaction processing. In this case, the median value might not be robust, since the quorum can consist of $f$ Byzantine values and more than one exceptionally low value.

            \end{itemize}

        \end{enumerate}



        \item If the leader is malicious:\\In this case, the median might not be robust. The reason is the leader can wait until it collects all CHECKPOINT messages, and then pick the faulty ones (measurement from slow honest nodes and Byzantine nodes) to assemble the quorum. We acknowledge this case might lead to an adversarial example in the inference or training phase, which might misguide the learning agent to choose a poorly performing architecture. However, in a homogeneous network, even when the leader is malicious, the median is robust. 

    \end{enumerate}

    Ensuring the robustness of the median values in the presence of node heterogeneity is an avenue for future work.
    Due to space limitations, we will include the complete discussion above in our extended technical report.

        
    \item \textbf{Minor point 1. You use the terms XOV, OXII in page 1 without explaining what they mean.}

    \hspace{8pt} Thank you for pointing them out. We have fixed them in {\bf \color{blue}Section~\ref{sec:intro}}.

    \item \textbf{Minor point 2. Page 3: unclear what "does not require an MVCC validation phase" means.}

    \hspace{8pt} Thank you for pointing it out. We replace the abbreviation with the full term in {\bf \color{blue}Section~\ref{sec:blockchain_arch_analysis}}.
    


\end{itemize}

\medskip
\noindent
{\large \textbf{Reviewer 2}}

\begin{itemize}
    \item \textbf{C1. The motivation of reinforcement learning is unclear to me. I understand that choosing the right blockchain will significantly accelerate the execution process. However, is it possible to use a relatively simple heuristic that is aware of workload characteristics and hardware features to determine the right blockchain architecture? As such, the learning overhead is minimized. }

    \hspace{8pt} We appreciate the suggestion that the motivation of reinforcement learning needs to be better elaborated. At a high level, reinforcement learning (RL) provides significant \textit{operational benefits }compared to crafting heuristics manually.

    \hspace{8pt} First, designing a good heuristic is difficult and cumbersome in the case of permissioned blockchains. For example, Hyperledger Fabric~\cite{androulaki2018hyperledger} has proposed that ``when the contention level is high, use OX; otherwise, use XOV''. Unfortunately, such a simple heuristic leads to wrong decisions in $50\%$ of our recorded traces, which results in poor performance and is likely going to be worse in a real BaaS production environment. This example suggests, to develop a good heuristic, an expert needs to exhaustively experiment over the entire state and action space to understand the intricate interactions. The expert also needs to carefully tune the specific threshold parameters that distinguish ``very high contention'' from ``high contention'', or ``low write ratio'' from ``moderate write ratio'', etc. Given the large space of workload (i.e., write ratio, contention level, load, compute intensity) and hardware features (i.e., CPU frequency and number of cores, RAM size, disk type and RPM, network latency and bandwidth), even if the expert discretizes each dimension by uniformly sampling $5$ points in it and tests each architecture for $5$ seconds, it takes {\em at least 90 days} to conduct the experiments even when the effect of block size is ignored\footnote{This back-of-the-envelope calculation works as below. The workload and hardware features have $8$ dimensions in total, resulting in $5^8$ combinations. Thus, it takes $5^8* 4*5$ seconds ($\approx 90.4$ days) to conduct the experiment.  }. 
    This is a conservative estimate given that most dimensions will require more than 5 sample points in practice.
    Due to the lack of blockchain simulators that capture the variations in architectures, such experiments are hard to be conducted in parallel.

    \hspace{8pt} Moreover, such heuristics are easily outdated when new hardware emerges or new blockchain architectures are introduced in the BaaS.  It could become very difficult for the expert to keep up with the new trend. For instance, when the BaaS provider introduces non-volatile RAM~\cite{tsai2020disaggregating} to replace the traditional combination of volatile RAM and disk, or when BaaS transitions to disaggregated architecture~\cite{wu2022flexchain} where there is extra latency for accessing memory, new hardware features are also naturally introduced.
    Thus, the expert needs to rerun all the performance profiling measurements over these new hardware to understand how they interact with workloads and blockchain architectures. Reinforcement learning removes the need for this entirely, since the system will optimize itself to whatever hardware and blockchain architectures at hand. In practice, if one has the human and compute resources to design an expert heuristic every time, doing so could potentially outperform our RL-based solution. However, we think this is not realistic for BaaS settings.

    \hspace{8pt} Last but not least, reinforcement learning does not incur additional overhead as compared to heuristics: as described in Section~\ref{sec:switching}, the training and inference required by learning are hidden due to the use of low watermark. Although reinforcement learning incurs some explorations in the action space, it is more acceptable than having inaccurate heuristics which are stuck at bad architectures. 
    
    \hspace{8pt}  We have significantly rewrite {\bf \color{blue}  Section~\ref{sec:case_for_adapt}} to better motivate reinforcement learning.


    
    
    
    \item \textbf{C2. The insight for the adaptation to different hardware is more needed. I understand that different hardware has different features that are friendly to different blockchain architectures. However, the corresponding insight is still missing. I think readers will prefer to see more details and insights.}

    \hspace{8pt} Thanks for pointing out this gap in the original submission. We have provided the readers with more insights on hardware's impact on architectures in {\bf \color{blue}Section~\ref{sec:blockchain_arch_analysis}}.
    

    \item \textbf{Minor point 1. The figures 2 and 3 are too small to read clearly.}

    \hspace{8pt} Thank you for pointing this out. Due to space limit, we will include enlarged version of Figures 2 and 3 in our extended technical report.
    

    
\end{itemize}

\medskip
\noindent
{\large \textbf{Reviewer 3}}

\begin{itemize}
    \item \textbf{W1. The paper's main contribution can be divided into two parts: predicting what configuration is best for the current workload, and a migration strategy. These two problems are well studied in the DB and systems literature. The paper needs to motivate more why this new context (permissioned blockchain) leads to new challenges or novelty in the problem. Alternatively, how is the proposed framework and algorithms different and contribute to the existing space of these two problems.}

    \hspace{8pt} We appreciate the suggestion of comparing to existing DB and system literature. \sys is inspired by previous work on learned databases~\cite{bao, neo, ml_index, selfdrivingcidr} and database migration~\cite{elmore2011zephyr, das2011albatross, kang2022remus, lin2019mgcrab, cao2022polardb}. However, permissioned blockchains is a unique application that requires: (1) unique featurization of the blockchain design landscape (i.e., action space); (2) fully decentralized machine learning including data collection, training, and inference, due to the untrustworthiness of blockchain participants; (3) migration in a safe manner that is robust to Byzantine failures; (4) migration in an efficient manner that mitigates the architecture exploration performed by reinforcement learning. Last but not least, unlike existing work that mainly migrates data between different physical nodes, \sys switches between system architectures within the same participating node. We have updated {\bf \color{blue}Section~\ref{sec:related}} to reflect the changes.



    \item \textbf{W2. I wonder what are the implications of this work (and problem space) in permissioned blockchains. Specifically. switching between configurations and protocols adds new risks for byzantine nodes to take malicious actions. This needs to be discussed in the paper as a complexity that may arise.}

    \hspace{8pt} We appreciate the suggestion of discussing the new threats introduced by architecture switching. We have added a {\bf \color{blue}Section~\ref{sec:security}} to present the threat model and discuss how \sys addresses those threats. 
    
    
    \item \textbf{W3. Another threat that may be introduced by the complexity of configuration and migration is a new attack vector. This new attack vector is to influence the workload to trigger a certain change in the system. This also needs a discussion. This can be combined with the risk of the previous point in the following way. The resilience of the system is reduced because the opportunity of attacking becomes not of finding an attack on one protocol, but rather in one of the n implemented protocols. Then, with the point made in the comment, an attacker may influence the workload to make the change into the least resilient protocol for an attack.}

    \hspace{8pt} We agree with the reviewer that when switching between architectures, the correctness guarantee becomes as strong as the weakest architecture in our action space. We have discussed this in {\bf \color{blue}Section~\ref{sec:security}}.
    
    \hspace{8pt} As a mitigation, we can test the correctness of the chosen set of architectures in advance, by using automated Byzantine fault generators such as the Twins tool~\cite{bano2022twins}. Once safety/liveness violations are discovered, we can exclude that architecture from our action space while still achieving adaptivity with other robust architectures. If no violations are discovered even using such an effective tool, the attacker is unlikely to know which architecture is non-resilient or which specific direction to influence the workload. 

        
    \item {\bf W4.  Instead of a lot of exploration in the CMAB solution, is it possible to provide some hints to the learning framework so that the learning and exploration processes are more efficient? Why or why not would be a good discussion to add.}

    \begin{figure*}
    \begin{minipage}{0.4\textwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figures/rsp_a_hint.png}
        \vspace{-2.2em}
        \captionsetup{format=plain, font=scriptsize}
        \caption*{\normalfont \,\,\,\,\, (a) Workload A}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figures/rsp_b_hint.png}
        \vspace{-2.2em}
        \captionsetup{format=plain, font=scriptsize}
        \caption*{\normalfont \,\,\,\,\, (b) Workload B}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figures/rsp_c_hint.png}
        \vspace{-2.2em}
        \captionsetup{format=plain, font=scriptsize}
        \caption*{\normalfont \,\,\,\,\, (c) Workload C}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figures/rsp_d_hint.png}
        \vspace{-2.2em}
        \captionsetup{format=plain, font=scriptsize}
        \caption*{\normalfont \,\,\,\,\, (d) Workload D}
    \end{minipage}
    \caption{\sys with hint.}
    \label{fig:hint}
    \end{figure*}

    \hspace{8pt} We appreciate the suggestion of discussing the possibility of providing hints. An expert administrator can build his knowledge into the learning framework by specifying certain rules in order to prevent exploring some sub-optimal decisions. An example hint is ``if the compute-intensity is higher than $2000$ us, enable early execution; otherwise, disable early execution". Hints of this nature reduce the architecture search space, thus providing faster convergence and avoiding certain explorations. Figure~\ref{fig:hint} summarizes our findings using the example hint (see ``AdaChain+hint'' on all graphs). For workload \A, the hint accelerates the convergence time of \sys by $3.8\times$. However, it is not sufficient to avoid all explorations in \sys,  i.e., varying reordering choice and block size. On the contrary, for workloads \B and \C where the convergence is already fast without the hint, the additional hint helps to reduce unnecessary explorations after convergence. Overall, our results on using correct hints are promising. 
    
    \hspace{8pt} However, a bad hint caused by inaccurate human knowledge can result in the exclusion of the optimal architectures. For example, if the administrator adjusts the hint above to be ``if the compute intensity is higher than 100 us, enable early execution; otherwise, disable early execution", \sys fails to converge to optimal on workload \B. We have updated {\bf \color{blue}Figure~\ref{fig:static} and Section~\ref{sec:expstatic}} to reflect the discussion above. 


    \item \textbf{W5. The framework formulation optimizes throughput. In a byzantine environment, is this the right metric to optimize? Even if not, is it right to optimize it in isolation of all other metrics? For instance, I would assume that "fairness" in terms of ensuring that transactions are not being unfairly delayed/dropped would be an interest since a leader (that is fast) might still be malicious by dropping/delaying some transactions.}

    \hspace{8pt} We completely agree with the reviewer that optimizing one metric might not be enough for all users.
    In \sys, we focus on effective throughput since it is the common metric used by previous benchmark tools~\cite{dinh2017blockbench, hyperledgercaliper, gramoli2022diablo} and literatures that proposed the fixed blockchain architectures~\cite{androulaki2018hyperledger, sharma2019blurring, ruan2020transactional, amiri2019parblockchain}.
    Latency or, as you mentioned, fairness are other good choices to consider or even combine with the current optimization goal (i.e., throughput).
    Regarding fairness, it should be noted that order-fairness is mainly about the ordering phase when the utilized consensus protocol needs to be fair (in contrast to \sys that targets transaction processing architecture). Since \sys uses a predefined consensus protocol for the ordering phase, using a fair protocol, e.g., Themis~\cite{kelkar2021themis} in \sys might address fairness attacks on the system.
    We plan to study extending the optimization goal to a combination of metrics as future work, where constrained optimization techniques are of interest. We have updated  {\bf \color{blue}Section~\ref{sec:learningalgo} ``AdaChain's formulation" sub-heading} to provide the justification.
    
    
    
    \item \textbf{W6. It is not clear how learning agents avoid malicious learning agents from influencing the learning or decision process. In section 3, there was a brief mention in step 3 about agents sharing with others to ensure that honest nodes are not influenced by dishonest nodes. However, how is this happening and how does the learning agent know which measurements are shared from honest or dishonest agents? similarly, it is not clear how everyone agrees on the same new protocol rather that some nodes making different decisions.}

    \hspace{8pt} We thank the reviewer for this comment, and agree that Section~\ref{sec:overview} was unclear on this point. Since the details on decision making are provided later in Section~\ref{sec:switching} and Section~\ref{sec:security}, we have updated {\bf \color{blue}step 3 in Section~\ref{sec:overview}} with a pointer to the later sections that include the details. Below, we answer the two questions raised in this comment.

    \begin{enumerate}
        \item The details are described in Algorithm~\ref{alg:regularpath}. Specifically, each node multicasts a CHECKPOINT message that includes its local measurement $e_i^{n+1}$ and $p_i^n$ to all other servers. Once the current leader collects a quorum $Q$ of $2f+1$ CHECKPOINT messages, it takes the median of all collected measurements to be the global state $e^{n+1}$ and global reward $p^n$. The leader then multicasts a PROPOSE message to all servers, which includes $e^{n+1}$, $p^n$ and the set $C$ of $2f+1$ received CHECKPOINT messages as the proof. Upon receiving the PROPOSE message, each node validates the message using set $C$, and goes through a PBFT-style protocol (lines 9-15) to commit the globally agreed measurement $e^{n+1}$ and $p^n$.

        \hspace{8pt} During this process, the dishonest nodes can only influence other honest nodes by reporting false measurements that deviate from the honest measurements. However, large deviations are prevented, since we use the median value as the global measurement and \sys is designed to operate in a homogeneous environment: if the $f$ dishonest nodes report false local measurements that are outliers (e.g., infinity or zero), they will be effectively ignored by computing the median. There is a possibility that a clever adversary could subtly influence the training process, potentially attacking the performance (but not correctness) of the system. This potential attack is discussed in Section~\ref{sec:security}.

        \item First, every honest node agrees on the same new architecture in the same episode. In \sys, each node's learning agent starts with the same random seed when it is launched. Thus, since both the state and reward of a certain episode are the same across all honest nodes (as mentioned in Section~\ref{sec:switching} and ~\ref{sec:security}), with the predictive model's deterministic training and inference, each honest agent chooses the same blockchain architecture in the same episode.  

        \hspace{8pt} Second, dishonest nodes can make decisions that are different from what honest nodes choose within the same episode. However, they can not affect the agreement on architecture among honest nodes, as we will show below: without loss of generality, we assume $f=1$ and there are $3f+1$ peers in the system, where $P_1, P_2, P_3$ are honest and $P_4$ is malicious; we assume the honest peers choose the XOV architecture.
        
        \hspace{8pt} We begin with the cases where $P_4$ the leader in the consensus protocol.
        If $P_4$ chooses OX in the same episode, it will send out transaction proposals instead of endorsements in the ordering phase, so honest peers will detect this mismatch and initiate a view-change.
        If $P_4$ chooses XOV but with a batch size $b_4$ that is different from what honest learning agents have chosen, it does not affect the agreement.
        If $P_4$ chooses XOV with different batch sizes and uses different batch sizes for different peers (e.g., $b_{4, 1}$ for $P_1$, $b_{4, 2}$ for $P_2$, etc.), the honest peers will detect and reject these batches during consensus on batches and initiate a view-change.
        If $P_4$ chooses XOV but with an opposite reordering choice, since reordering happens locally on each peer according to its local model, the malicious peer cannot corrupt honest peers. None of the scenarios above affects the agreement.
        
        \hspace{8pt} In the cases where $P_4$ is not the leader in the consensus protocol, the honest leader can detect type mismatch for messages originating from $P_4$ and discard them, while other honest peers work as normal. We have added a {\bf \color{blue}Section~\ref{sec:security}} to reflect this discussion, and reorganized Section~\ref{sec:predictivemodel} accordingly.

    \end{enumerate}

    
    
    

    \item \textbf{W7. The use of Thompson sampling may pose a problem in terms of the security of the distributed system. It is well-studied that even safe and popular BFT protocols suffer from liveness and performance attacks. This makes it feasible for a malicious node(s) to influence Thompson sampling by selectively attacking the performance/liveness of the system during the sampling points that it wants to be avoided. This would enable a malicious node attack where the Thompson sampling is played. }

    \hspace{8pt} We agree with the reviewer that the security of Thompson sampling is an important aspect to discuss. We have added a {\bf \color{blue}Section~\ref{sec:security}} to reflect the discussion below.
    \begin{enumerate}
    
    
    \item \textbf{Correctness.} Most importantly, using Thompson sampling does not expose extra correctness concerns. The correctness of \sys only depends on the consensus protocol (which is predefined in our system), the current architecture, and our switching protocol. That being said, \sys's correctness guarantee is always as strong as the weakest architecture in its action space, regardless of the specific reinforcement learning algorithm.
    
    \item \textbf{Performance.} Thompson sampling introduces a new performance attack vector: misguiding the learning agent to pick a bad architecture according to the workload. A malicious node can certainly manipulate its local Thompson sampling process by avoiding/forging some points. However, since Thompson sampling is replicated on every node in \sys, it is not sufficient to disrupt the honest nodes into choosing a bad architecture. Instead, the malicious node needs to propose adversarial values into the quorum $Q$ in Algorithm~\ref{alg:regularpath}, in order to make such attacks effective. Specifically, there are at least two ways adversarial values could negatively impact performance:

    \begin{enumerate}
        \item \textbf{Decision attack.} This attack targets the inference phase of the machine learning pipeline. A malicious node reports a false observation of its local state $e_i^{n+1}$ in order to push the global state in one direction or another. 
        

        \item \textbf{Poisoning attack.} This attack targets the training phase of the machine learning pipeline. Since the malicious nodes know details about the predictor $M_{\theta}$ (i.e., random forest), they can report carefully selected (e.g., slightly biased) local states $e_i^{n+1}$ and rewards $p_i^n$, which accumulate in the experience buffer and lead to an inaccurate $M_{\theta}$ being trained. 
        

    \end{enumerate}
    
    \sys mitigates such attacks by selecting the median value of all reported features. For a feature with low variance, adversaries would only be able to move the median value by a small amount even if they can report strong outliers (e.g., infinity or zero). However, for a feature with high variance, adversaries could potentially create a non-trivial change in the median value, impacting future inference and training. Since \sys is designed to operate in a homogeneous environment, most existing features and labels have low variance.
    We flag studying the full impact of adversarial learning~\cite{goodfellow2014explaining, kurakin2016adversarial, madry2018towards, wong2019fast} on a system like \sys as potential future work.
    \end{enumerate}

    

        
\end{itemize}
			

\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{0}
